CPlaNet: Enhancing Image Geolocalization by Combinatorial Partitioning of Maps

Image geolocalization is the task of identifying the location depicted in a photo based only on its visual information. This task is inherently challenging since many photos have only few, possibly ambiguous cues to their geolocation. Recent work has cast this task as a classification problem by partitioning the earth into a set of discrete cells that correspond to geographic regions. The granularity of this partitioning presents a critical trade-off; using fewer but larger cells results in lower location accuracy while using more but smaller cells reduces the number of training examples per class and increases model size, making the model prone to overfitting. To tackle this issue, we propose a simple but effective algorithm, combinatorial partitioning, which generates a large number of fine-grained output classes by intersecting multiple coarse-grained partitionings of the earth. Each classifier votes for the fine-grained classes that overlap with their respective coarse-grained ones. This technique allows us to predict locations at a fine scale while maintaining sufficient training examples per class. Our algorithm achieves the state-of-the-art performance in location recognition on multiple benchmark datasets.

==> ECCV 2018 (CP) Camera Ready/sections/abstract.tex <==
% !TEX root = ../main.tex

\begin{abstract}
%
Image geolocalization is the task of identifying the location depicted in a photo based only on its visual information. 
This task is inherently challenging since many photos have only few, possibly ambiguous cues to their geolocation.
Recent work has cast this task as a classification problem by partitioning the earth into a set of discrete cells that correspond to geographic regions.
The granularity of this partitioning presents a critical trade-off; using fewer but larger cells results in lower location accuracy while using more but smaller cells reduces the number of training examples per class and increases model size, making the model prone to overfitting.
%
To tackle this issue, we propose a simple but effective algorithm, combinatorial partitioning, which generates a large number of fine-grained output classes by intersecting multiple coarse-grained partitionings of the earth.
%
Each classifier votes for the fine-grained classes that overlap with their respective coarse-grained ones. 
This technique allows us to predict locations at a fine scale while maintaining sufficient training examples per class.
%
Our algorithm achieves the state-of-the-art performance in location recognition on multiple benchmark datasets.
%
\keywords{Image geolocalization, combinatorial partitioning, fine-grained classification}
\end{abstract}

==> ECCV 2018 (CP) Camera Ready/sections/comb_part.tex <==
% !TEX root = ../main.tex

%%%%%%%%% BODY TEXT
\section{Geolocalization using Multiple Classifiers}
\label{sec:comb_part}

%\hsseo{(Overall description of the method)}
Unlike existing classification-based methods~\cite{weyand16planet}, CPlaNet relies on multiple classifiers that are all trained with unique geoclass sets.
%\footnote{Our approach is distinguished from simple ensemble methods because each model is learned with a unique set of classes.}.
The proposed model predicts more fine-grained geoclasses, which are given by combinatorial partitioning of multiple geoclass sets.
%By combinatorially merging the results of these classifiers, our model obtains scores over more finely divided regions than those of the geo-classes for each classifier.
Since our method requires a distinct geoclass set for each classifier, we also propose a way to generate multiple geoclass sets.

\iffalse
\subsection{Geolocalization by Classification}
%\hsseo{(review of classification based model)}
We briefly review the classification based geolocalization methods.
In~\cite{vo17revisiting,weyand16planet}, a classifier is trained to predict the geolocation of an input image.
Since the geolocation is represented in a continuous space, the authors introduce a geoclass set that quantizes the maps of the entire earth by partitioning it into regions.
Note that training images are labeled with the corresponding geoclass based on their GPS tags.
At test time, the center of the geoclass with the highest score is returned as the predicted geolocation of an input image.
This method is computationally cheap in terms of space and time complexity compared to retrieval-based methods, but its quality is highly dependent on how the geoclass set is generated.
Since every image that belongs to the same geoclass has an identical predicted geolocation, more fine-grained partitioning is preferable to obtain precise predictions.
However, it is not always straightforward to increase the number of geoclasses as it linearly increases the number of parameters and makes the network prone to overfitting to training data.
\fi

\subsection{Combinatorial Partitioning}
\label{sec:sub:part}
%\hsseo{(Our method)}
\iffalse
We propose a novel classification-based geolocalization model using a combination of multiple geoclass sets.
Unfortunately, there is no standard method to define geoclasses for image geolocalization and an arbitrary choice may incur undesirable artifacts.
We alleviate this limitation by diversifying geoclass sets; we construct multiple distinct geoclass sets by applying different partitioning criteria.
\fi
Our primary goal is to establish fine-grained geoclasses through a combination of multiple coarse geoclass sets and exploit benefits from both coarse- and fine-grained geolocalization-by-classification approaches.
In our model, there are multiple unique geoclass sets represented by partitions $\mathcal{P}=\{p_1,p_2,\dots,p_5\}$ and $\mathcal{Q}=\{q_1,q_2,\dots,q_5\}$ as illustrated on the left side of Figure~\ref{fig:comb_part}.
Since the region boundaries in these geoclass sets are unique, overlapping the two maps constructs a set of fine-grained subregions.
This procedure, referred to as combinatorial partitioning, is identical to the Cartesian product of the two sets, but disregards the tuples given by two spatially disjoint regions in the map.
%; a subpartition is generated as a tuple of partitions from each geoclass set.
For instance, combining two aforementioned geoclass sets in Figure~\ref{fig:comb_part}, we obtain fine-grained partitions defined by a tuple $(p_i, q_j)$ as depicted by the map on the right of the figure, while the tuples made by two disjoint regions, {\it e.g.,} $(p_1, q_5)$, are not considered.
%Note that the region boundaries among the geoclass sets are unique and a region in a geoclass set is subdivided by another set resulting in more fine-grained partitions as depicted by the map on the top of Figure~\ref{fig:comb_part}.
%In our model, there are $N$ unique geoclass sets as illustrated at the bottom of Figure~\ref{fig:comb_part}.
%Note that the region boundaries among all geoclass sets are unique and a region in a geoclass set is subdivided by another set resulting in more fine-grained partitions as depicted by the map on the top of Figure~\ref{fig:comb_part}.
%{\color{red} [Rewrite this paragraph in a more technical way based on the updated figure.]}

%This process is related to an ensemble method with voting at inference time, 
While combinatorial partitioning aggregates results from multiple classifiers, it is conceptually different from ensemble models whose base classifiers predict labels in the same output space.
In combinatorial partitioning, while each coarse-grained partition is scored by a corresponding classifier, fine-grained partitions are given different scores by the combinations of multiple unique geoclass sets.
Also, combinatorial partitioning is closely related to product quantization~\cite{jegou11product} for approximate nearest neighbor search in the sense that they both generate a large number of quantized regions by either a Cartesian product of quantized subspaces or a combination of coarse space quantizations. 
Note that combinatorial partitioning is a general framework and applicable to other tasks, especially where labels have to be defined on the same embedded space as in geographical maps.



% Some good points of our method:
%   1) Needs less parameters for the same number of distinct regions
%   2) A region is grouped with different regions together that may share different visual features
%   3) If we divide regions into very fine regions, there will be lack of training examples for each class
\subsection{Benefits of Combinatorial Partitioning}
\label{sec:sub:benefits}
%A straightforward way to obtain a fine-grained partition is to increase the number of geoclasses within a single set.
The proposed classification model with combinatorial partitioning has the following three major benefits.

%\vspace{-0.4cm}
\subsubsection{Fine-grained classes with fewer parameters}
Combinatorial partitioning generates fine-grained geoclasses using a smaller number of parameters because a single geoclass in a class set can be divided into many subregions by intersections with geoclasses from multiple geoclass sets.
For instance in Figure~\ref{fig:comb_part}, two sets with 5 geoclasses form 14 distinct classes by the combinatorial partitioning.
If we design a single flat classifier with respect to the fine-grained classes, it requires more parameters, \ie, $14 \times F > 2\times(5\times F)$, where $F$ is the number of input dimensions to the classification layers.
%\brk{If we design a single classifier with the same number of parameters, \ie $2 \times(5 \times F) = 10 \times F$, where $F$ is the number of input dimensions to the classification layers, it only has 10 distinct classes.}
\iffalse
\brk{The naive approach requires significantly more parameters in the classification layer than combinatorial partitioning given the same number of geoclasses---after the combination in our algorithm.
Note that our combinatorial partitioning generates more geoclasses with the same number of parameters because a single geoclass in a class set can be divided into many subregions by intersections of geoclasses in multiple geoclass sets.
For instance, in Figure~\ref{fig:comb_part}, two sets with 5 geoclasses form 14 distinct classes by the combinatorial partitioning, while the network made by a naive partitioning has only 10 distinct classes.}
Note that both cases require the same number of parameters, \ie, $2 \times(5 \times F) = 10 \times F$ where $F$ is the number of input dimensions to the classifiers.
\fi

%\vspace{-0.4cm}
\subsubsection{More training data per class}
Training with fine-grained geoclass sets is more desirable for higher resolution of output space, but is not straightforward due to training data deficiency; the more we divide the maps, the less training images remain per geoclass.
Our combinatorial partitioning technique enables us to learn models with coarsely divided geoclasses and maintain more training data in each class than a na\"ive classifier with the same number of classes.

%Since the proposed model learns can generate a large number of geoclasses through combinatorial partitioning, it requires to learn the model with a smaller geoclass set than the naive method in each classifier.
%On the other hand, the proposed model never reduces the number of training examples per geoclass in existing geoclass sets; 
%instead generates a new geoclass set that can take the aforementioned advantages.

%\vspace{-0.4cm}
\subsubsection{More reasonable class sets}
There is no standard method to define geoclasses for image geolocalization, so that images associated with the same classes have common characteristics.
%and associate the defined labels with geographical regions.
An arbitrary choice of partitioning may incur undesirable artifacts due to heterogeneous images located near class territories; the features trained on loosely defined class sets tend to be insufficiently discriminative and less representative.
%In practice, arbitrary criteria may be employed to generate class sets, which leads heterogeneous images to reside within the territory of a class.
On the other hand, our framework constructs diverse partitions based on various criteria observed in the images. 
We can define more tightly-coupled classes through combinatorial partitioning by distilling noisy information from multiple sources.


\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.31\linewidth}
\centering
\includegraphics[width=1\linewidth] {./figures/geoclasses/classset1.pdf}
\vspace{-0.23in}
\caption{Geoclass set 1}
\end{subfigure}
~~
\begin{subfigure}[t]{0.31\linewidth}
\centering
\includegraphics[width=1\linewidth] {./figures/geoclasses/classset2.pdf}
\vspace{-0.23in}
\caption{Geoclass set 2}
\end{subfigure}
~~
\begin{subfigure}[t]{0.31\linewidth}
\centering
\includegraphics[width=1\linewidth] {./figures/geoclasses/classset3.pdf}
\vspace{-0.23in}
\caption{Geoclass set 3}
\end{subfigure}

\vspace{0.08in}

\begin{subfigure}[t]{0.31\linewidth}
\centering
\includegraphics[width=1\linewidth] {./figures/geoclasses/classset4.pdf}
\vspace{-0.23in}
\caption{Geoclass set 4}
\end{subfigure}
~~
\begin{subfigure}[t]{0.31\linewidth}
\centering
\includegraphics[width=1\linewidth] {./figures/geoclasses/classset5.pdf}
\vspace{-0.23in}
\caption{Geoclass set 5}
\end{subfigure}
\caption{
Visualization of the geoclass sets on the maps of the United States generated by the parameters shown in Table~\ref{tab:geoclass}. 
Each distinct region is marked by a different color.
The first two sets, (a) and (b), are generated by manually designed parameters while parameters for the others are randomly sampled.
%{\color{red} [Convert the images to png format, which will make loading much faster.]}
}
\label{fig:class_set}
%\vspace{-0.1in}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

\begin{figure}[t]
\centering
\includegraphics[width=0.32\linewidth] {./figures/geoclasses/classset1.pdf}
\includegraphics[width=0.32\linewidth] {./figures/geoclasses/classset2.pdf} \\
\centerline{(a) Geoclass set 1 \quad\quad\quad\quad (b) Geoclass set 2}
\includegraphics[width=0.32\linewidth] {./figures/geoclasses/classset3.pdf}
\includegraphics[width=0.32\linewidth] {./figures/geoclasses/classset4.pdf}
\includegraphics[width=0.32\linewidth] {./figures/geoclasses/classset5.pdf}
\centerline{(c) Geoclass set 3 \quad\quad\quad\quad~ (d) Geoclass set 2 ~\quad\quad\quad\quad (3) Geoclass set 3}
\caption{
Visualization of the geoclass sets on the maps of the United States generated by the parameters shown in Table~\ref{tab:geoclass}. 
Each distinct region is marked by a different color.
The first two sets, (a) and (b), are generated by manually designed parameters while parameters for the others are randomly sampled.
%{\color{red} [Convert the images to png format, which will make loading much faster.]}
}
\label{fig:class_set}
%\vspace{-0.1in}
\end{figure}


\subsection{Generating Multiple Geoclass Sets}
\label{sec:sub:geo_gen}
%\hsseo{(Initial graph structure)}
The geoclass set organization is an inherently ill-posed problem as there is no consensus about ideal region boundaries for image geolocalization.
Consequently, it is hard to define the optimal class configuration, which motivates the use of multiple random boundaries in our combinatorial partitioning.
%As the proposed model requires multiple geoclass sets, w
We therefore introduce a mutable method of generating geoclass sets, which considers both visual and geographic distances between images.

The generation method starts with an initial graph for a map, where a node represents a region in the map and an edge connects two nodes of adjacent regions.
We construct the initial graph based on S2 cells\footnote{We use Google's S2 library. S2 cells are given by a geographical partitioning of the earth into a hierarchy. The surface of the earth is projected onto six faces of a cube. Each face of the cube is hierarchically subdivided and forms S2 cells in a quad-tree. Refer to \url{https://code.google.com/archive/p/s2-geometry-library/ for more details.}} at a certain level.
Empty S2 cells, which contain no training image, do not construct separate nodes and are randomly merged with one of their neighboring non-empty S2 cells.
This initial graph covers the entire surface of the earth.
Both nodes and edges are associated with numbers---scores for nodes and weights for edges.
% We score nodes by a linear combination of three different factors: the number of images in the node, the number of non-empty S2 cells, and the number of S2 cells (including empty cells).
We give a score to each node by a linear combination of three different factors: the number of images in the node and the number of empty and non-empty S2 cells.
%The non-empty S2 cells---after merging with empty S2 cells---form the initial nodes and any adjacent two regions are connected by an edge.
%We then define the cardinality of a node as a linear combination of three factors: the number of images in the node, the number of non-empty S2 cells and the number of S2 cells (including empty cells).
% We then define the cardinality {\color{red} [Cardinality sounds weird to me.]} of a node as a linear combination of the following three factors: the number of images, non-empty S2 cells and empty S2 cells in the node.
%{\color{red} [Cardinality sounds weird to me.]}
An edge weight is computed by the weighted sum of geolocational and visual distances between two nodes.
The geolocational distance is given by the distance between the centers of two nodes while the visual distance is measured by cosine similarity based on the visual features of nodes, which are computed by averaging the associated image features extracted from the bottleneck layer of a pretrained CNN.
%
Formally, a node score $\omega(\cdot)$ and an edge weight $\nu(\cdot, \cdot)$ are defined respectively as
%
\begin{align}
    \omega(v_i) &= \alpha_1 \cdot n_\mathrm{img}(v_i) + \alpha_2 \cdot n_\mathrm{S2+}(v_i) + \alpha_3 \cdot n_\mathrm{S2}(v_i) \\
    %\mathrm{NS}(n_i) &= \alpha\mathrm{\#img}(n_i) +\beta\mathrm{\#non\_empty}(n_i) + \gamma \mathrm{\#S2}(n_i) \\
    \nu(v_i, v_j) &= \beta_1 \cdot \mathrm{dist_{vis}}(v_i, v_j) + \beta_2 \cdot \mathrm{dist_{geo}}(v_i, v_j)
    %\mathrm{EW}(n_i, n_j) &= \zeta\mathrm{vis\_dist}(n_i, n_j) + \eta\mathrm{geo\_dist}(n_i, n_j)
\end{align}
%
where $n_\mathrm{img}(v)$, $n_\mathrm{S2+}(v)$ and $n_\mathrm{S2}(v)$ are functions that return the number of images, non-empty S2 cells and all S2 cells in a node $v$, respectively, and $\mathrm{dist_{vis}}(\cdot,\cdot)$ and $\mathrm{dist_{geo}}(\cdot, \cdot)$ are the visual geolocational distances between two nodes.
Note that the weights $(\alpha_1, \alpha_2, \alpha_3)$ and $(\beta_1, \beta_2)$ are free parameters in $[0, 1]$.


\begin{table}[t]
\centering
\caption{Parameters for geoclass set generation. 
Parameters for geoclass set 1 and 2 are manually given while the ones for rest geoclass sets are randomly sampled.}
%\vspace{-0.2cm}
\scalebox{0.9}{
\begin{tabular}{
@{}C{1.8cm}@{}|@{}C{6.1cm}@{}|@{}C{1.1cm}@{}@{}C{1.1cm}@{}|@{}C{1.1cm}@{}@{}C{1.1cm}@{}@{}C{1.1cm}@{}
}
\multicolumn{6}{l}{}\\
Parameter group                 & Parameters                                     & 1         & 2         & 3         & 4         & 5         \\ \hline\hline
\multirow{2}{*}{N/A}            & Num. of geoclasses                              & 9,969     & 9,969     & 12,977    & 12,333    & 11,262    \\ 
                                & Image feature dimensions                & 2,048     & 0         & 1,187     & 1,113     & 14,98     \\ \hline
\multirow{3}{*}{\parbox{1.8cm}{\centering Node score}}     & Weight for num. of images ($\alpha_1$)             & 1.000     & 1.000     & 0.501     & 0.953     & 0.713     \\ 
                                & Weight for num. of non-empty S2 cells ($\alpha_2$) & 0.000     & 0.000     & 0.490     & 0.044     & 0.287     \\ 
                                & Weight for num. of S2 cells ($\alpha_3$)          & 0.000     & 0.000     & 0.009     & 0.003     & 0.000     \\ \hline 
\multirow{2}{*}{\parbox{1.8cm}{\centering Edge weight}}    & Weight for visual distance ($\beta_1$)          & 1.000     & 0.000     & 0.421     & 0.628     & 0.057     \\ 
                                & Weight for geographical distance ($\beta_2$)    & 0.000     & 1.000     & 0.579     & 0.372     & 0.943     \\ \hline
\end{tabular}
}
\label{tab:geoclass}
\end{table}


%\hsseo{(Merge algorithm)}
After constructing the initial graph, we merge two nodes hierarchically in a greedy manner until the number of remaining nodes becomes the desired number of geoclasses.
To make each geoclass roughly balanced, we select the node with the lowest score first and merge it with its nearest neighbor in terms of edge weight.
A new node is created by the merge process and corresponds to the region given by the union of two merged regions.
The score of the new node is set to the sum of the scores of the two merged nodes.

%\hsseo{(parameters of this method for random generaton)}
The generated geoclass sets are diversified by the following free parameters: 1) the desired number of final geoclasses, 2) the weights of the factors in the node scores, 3) the weights of the two distances in computing edge weights and 4) the image feature extractor.
Each parameter setting constructs a unique geoclass set.
Note that multiple geoclass set generation is motivated by the fact that geoclasses are often ill-defined and the perturbation of class boundaries is a natural way to address the ill-posed problem.
Figure~\ref{fig:class_set} illustrates generated geoclass sets using different parameters described in Table~\ref{tab:geoclass}.




==> ECCV 2018 (CP) Camera Ready/sections/conclusion.tex <==
% !TEX root = ../main.tex

%%%%%%%%% BODY TEXT
\section{Conclusion}
\label{sec:conclusion}

We proposed a novel classification-based approach for image geolocalization, {referred to as CPlaNet}.
Our model obtains the final geolocation of an image using a large number of fine-grained regions given by combinatorial partitioning of multiple classifiers.
%Our model employs multiple classifiers and obtains the final geolocation using a fine-grained region given by combinatorial partitioning.
We also introduced an inference procedure appropriate for classification-based image geolocalization.
The proposed technique improves image geolocalization accuracy with respect to other methods in multiple benchmark datasets especially at fine scales, and also outperforms the individual coarse-grained classifiers.
%We also show that our method achieves the state-of-the-art performance at majority of scales over previous methods on the Im2GPS test set.

==> ECCV 2018 (CP) Camera Ready/sections/experiments.tex <==
% !TEX root = ../main.tex

%%%%%%%%% BODY TEXT
\section{Experiments}
\label{sec:exp}

\subsection{Datasets}
\label{sub:datasets}
We train our network using a private dataset collected from Flickr, which has 30.3M geotagged images for training. 
We have sanitized the dataset by removing noisy examples to weed out unsuitable photos. 
For example, we disregard unnatural images (e.g., clipart images, product photos, etc.) and accept photos with a minimum size of 0.1 megapixels.
%
%We train our network using a private dataset collected from Flickr, which has 30.3M geotagged images for training.
%This dataset contains a subset of images used for training the model for \cite{weyand16planet}; we have sanitized the original dataset by removing noisy examples to weed out unsuitable photos.
%For example, we disregard unnatural images (e.g., clipart images, product photos, etc.) and accept photos with a minimum size of 0.1 megapixels.
%For example, we accept images only if they look natural based on classifier outputs (e.g., non-clipart images, non-product photos, images with natural background) and have a minimum size of 0.1 megapixels. 

For evaluation, we mainly employ two public benchmark datasets---Im2GPS3k and YFCC4k~\cite{vo17revisiting}. 
The former contains 3,000 images from the Im2GPS dataset whereas the latter has 4,000 random images from the YFCC100m dataset.
In addition, we also evaluate on Im2GPS test set~\cite{hays08im2gps} to compare with previous work.
%, which consists of 237 Flickr photos manually selected to contain at least some geolocation cues.
Note that Im2GPS3k is a different test benchmark from the Im2GPS test set.

\iffalse
We introduce a new dataset called FlickrGeo, which consists of 44.8M geotagged photos from Flickr. 
FlickrGeo is split into 30.3M training images and 14.5M testing images, and contains images from all around the world. 
Minimal filtering has been applied to weed out unsuitable photos; we accept images only if they look natural based on classifier outputs (e.g., non-clipart images, non-product photos, images with natural background) and have a minimum size of 0.1 megapixels. 
Both dataset size and image distribution make this dataset challenging.
%
For comparability with previous work, we also evaluate on the Im2GPS test set~\cite{hays08im2gps} that consists of 237 Flickr photos manually selected to contain at least some geolocation cues.
\fi

\subsection{Parameters and Training Networks}
\label{sub:parameters}
We generate three geoclass sets using randomly generated parameters, which are summarized in Table~\ref{tab:geoclass}.
The number of geoclasses for each set is approximately between 10K and 13K, and the generation parameters for edge weights and node scores are randomly sampled.
%{\color{red}the weights for the factors in the cardinality and the edge weight are also randomly sampled.}
%Specifically, we select random axis-aligned subspaces out of the full 2,048 dimensions for image representations, and define diverse dissimilarity metrics between image representations.
Specifically, we select random axis-aligned subspaces out of the full 2,048 dimensions for image representations to diversify dissimilarity metrics between image representations.
%Note that we employ a reproduced PlaNet~\cite{weyand16planet} as our visual feature extractor for the geoclass set generation, after removing the final classification layer.
Note that the image representations are extracted by a reproduced PlaNet~\cite{weyand16planet} after removing the final classification layer.
In addition to these geoclass sets, we generate two more sets with manually designed parameters; the edge weights in these two cases are given by either visual or geolocational distance exclusively, and their node scores are based on the number of images to mimic the setting of PlaNet.
Figure~\ref{fig:class_set} visualizes five geoclass sets generated by the parameters presented in Table~\ref{tab:geoclass}.

We use S2 cells at level 14 to construct the initial graph, where a total of $\sim$2.8M nodes are obtained after merging empty cells to their non-empty neighbors.
%\hsseo{Note that the numbers of initial S2 cells and nodes are already large and thus the greedy strategy in our geoclass set generation is beneficial regarding the time complexity.}
%
To train the proposed model, we employ the pretrained model of the reproduced PlaNet with its parameters fixed while the multiple classification branches are randomly initialized and fine-tuned using our training dataset.
The network is trained by RMSprop with a learning rate of 0.005.


\subsection{Evaluation Metrics}
Following \cite{vo17revisiting,weyand16planet}, we evaluate the models using geolocational accuracies at multiple scales by varying the allowed errors in terms of distances from ground-truth locations as follows: 1~km, 5~km, 10~km, 25~km, 50~km, 100~km, 200~km, 750~km and 2500~km.
Our evaluation focuses more on high accuracy range compared to the previous papers as we believe that fine-grained geolocalization is more important in practice.
A geolocational accuracy $a_r$ at a scale is given by the fraction of images in the test set localized within radius $r$ from ground-truths, which is given by
%Following \cite{vo17revisiting,weyand16planet}, we evaluate the models using geolocational accuracies at the following five scales in terms of radius, distance to ground-truth location: street (1~km), city (25~km), region (200~km), country (750~km), and continent (2500~km).
%
\begin{equation}
\label{eq:geo_acc}
a_r\equiv\frac{1}{M}\sum_{i=1}^{M}{u\left[ \mathrm{geodist}\left(l_\mathrm{gt}^i, l_\mathrm{pred}^i\right) < r \right]},
\end{equation}
%
where $M$ is the number of examples in the test set, $u[\cdot]$ is an indicator function and $\mathrm{geodist}(l_\mathrm{gt}^i, l_\mathrm{pred}^i)$ is the geolocational distance between the true image location $l_\mathrm{gt}^i$ and the predicted location $l_\mathrm{pred}^i$ of the $i$-th example.




\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\caption{Geolocational accuracies [\%] of models at five different scales on FlickrGeo.}
\label{tab:flickrgeo}
\scalebox{0.9}{
\begin{tabular}{
p{2.3cm}@{}|@{}C{1.3cm}@{}@{}C{1.3cm}@{}@{}C{1.35cm}@{}@{}C{1.45cm}@{}@{}C{1.65cm}@{}
}
Models	                        & Street 1~km	& City 25~km	& Region 200~km	& Country 750~km    & Continent 2500~km	\\ \hline\hline
ImageNetFeat	                & 1.5           & \phantom{0}3.4& \phantom{0}6.9& 17.6              & 37.7          	\\
% PlaNet~(reprod)                 & 3.7           & 12.0          & 22.5          & 38.9              & 58.5          	\\ \hline
PlaNet~(reprod)                 & 4.5           & 12.0          & \bf{21.3}     & \bf{37.4}         & \bf{56.8}      	\\ \hline
%PlaNet                          & 4.5           & 12.0          & 21.3          & \bf{37.4}         & \bf{56.8}      	\\ \hline
ClassSet~1	                    & 4.8           & 11.6          & 20.6          & 36.9              & 56.5          	\\
ClassSet~2	                    & 4.3           & 11.7          & 20.5          & 36.8              & 56.4       	    \\
ClassSet~3	                    & 4.8           & 12.1          & 20.8          & 37.1              & 56.6          	\\
ClassSet~4	                    & 5.0           & 11.8          & 20.7          & 37.0              & 56.6          	\\
ClassSet~5	                    & 4.7           & 11.9          & 20.7          & 37.0              & 56.5          	\\ \hline
Average[1-2]	                & 4.6           & 11.6          & 20.6          & 36.8              & 56.5          	\\
Average[1-5]                    & 4.7           & 11.8          & 20.7          & 36.9              & 56.5          	\\ \hline
%Max[1-2]    	                & 4.8           & 11.7          & 20.6          & 36.9              & 56.5          	\\
%Max[1-5]                        & 5.0           & 12.1          & 20.8          & 37.1              & 56.6          	\\ \hline
%SingleSet (1-2)	                & 5.5           & 11.8          & 20.4          & 36.4              & 56.1          	\\
%SingleSet (1-5)                 & ---           & ----          & ----          & ----              & ----          	\\ \hline
CP[1-2] 	                & 5.5           & 12.2          & 20.9          & 37.1              & 56.6          	\\
CP[1-5]                   & 5.8           & 12.4          & 21.1          & 37.2              & 56.7          	\\ 
CP[1-5,PlaNet]                 & \bf{6.1}      & \bf{12.6}     & \bf{21.3}     & 37.3              & \bf{56.8}         \\
\hline
\end{tabular}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\caption{Geolocational accuracies [\%] of models at different scales on Im2GPS3k.}
\label{tab:im2gps3k}
\scalebox{0.9}{
\begin{tabular}{
p{3.1cm}@{}|@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.5cm}@{}
}
Models                                  & 1~km      & 5~km      & 10~km	    & 25~km     & 50~km     & 100~km    & 200~km    & 750~km    & 2500~km   \\ \hline\hline
ImageNetFeat                            & 3.0       & 5.5       & 6.4       & 6.9       & 7.7       & 9.0       & 10.8      & 18.5      & 37.5      \\ \hline
Deep-Ret~\cite{vo17revisiting}          & 3.7       & --        & --        & 19.4      & --        & --        & 26.9      & 38.9      & 55.9      \\
PlaNet~(reprod)~\cite{weyand16planet}   & 8.5       & 18.1      & 21.4      & 24.8      & 27.7      & 30.0      & 34.3      & 48.4      & \bf{64.6} \\ \hline
ClassSet~1                              & 8.4       & 18.3      & 21.7      & 24.7      & 27.4      & 29.8      & 34.1      & 47.9      & 64.5      \\
ClassSet~2                              & 8.0       & 17.6      & 20.6      & 23.8      & 26.2      & 29.2      & 32.7      & 46.6      & 63.9      \\
ClassSet~3                              & 8.8       & 18.9      & 22.4      & 25.7      & 27.9      & 29.8      & 33.5      & 47.8      & 64.1      \\
ClassSet~4                              & 8.7       & 18.5      & 21.4      & 24.6      & 26.8      & 29.6      & 33.0      & 47.6      & 64.4      \\
ClassSet~5                              & 8.8       & 18.7      & 21.7      & 24.7      & 27.3      & 29.3      & 32.9      & 47.1      & 64.5      \\ \hline
Average[1-2]                            & 8.2       & 18.0      & 21.1      & 24.2      & 26.8      & 29.5      & 33.4      & 47.3      & 64.2      \\
Average[1-5]                            & 8.5       & 18.4      & 21.5      & 24.7      & 27.1      & 29.5      & 33.2       & 47.4      & 64.3      \\ \hline
CPlaNet[1-2]                                 & 9.3       & 19.3      & 22.7      & 25.7      & 27.7      & 30.1      & 34.4      & 47.8      & 64.5      \\
CPlaNet[1-5]                                 & 9.9       & 20.2      & 23.3      & 26.3      & 28.5      & 30.4      & 34.5      & \bf{48.8} & \bf{64.6} \\ 
CPlaNet[1-5,PlaNet]                          & \bf{10.2} & \bf{20.8} & \bf{23.7} & \bf{26.5} & \bf{28.6} & \bf{30.6} & \bf{34.6} & 48.6      & \bf{64.6} \\
\hline
\end{tabular}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\subsection{Results}

%\subsubsection*{5.4.1 Benefits of Combinatorial Partitioning \vspace{0.3cm} \\ }
\subsubsection{Benefits of Combinatorial Partitioning}

Table~\ref{tab:im2gps3k} presents the geolocational accuracies of the proposed model on the Im2GPS3k dataset.
The proposed models outperform the baselines and the existing methods at almost all scales on this dataset.
ClassSet~1 through 5 in Table~\ref{tab:im2gps3k} are the models trained with the geoclass sets generated from the parameters presented in Table~\ref{tab:geoclass}.
Using the learned models as the base classifiers, we construct two variants of the proposed method---{CPlaNet}[1-2] using the first two base classifiers with manual parameter selection and CPlaNet[1-5] using all the base classifiers.
% where CP denotes combinatorial partitioning.

Table~\ref{tab:im2gps3k} presents that both options of our models outperform all the underlying classifiers at every scale.
Compared to na\"ive average of the underlying classifiers denoted by Average[1-5] and Average[1-2], {CPlaNet}[1-5] and {CPlaNet}[1-2] have $\sim$16 \% and $\sim$13 \% of accuracy gains at street level, respectively, compared to their counterparts.
We emphasize that {CPlaNet} achieves substantial improvements by a simple combination of the existing base classifiers and a generation of fine-grained partitions without extra training procedure.
%This means that the geolocalization quality is improved through the combination process of merging individual results into fine-grained partitions.
The larger performance improvement in {CPlaNet}[1-5] compared to {CPlaNet}[1-2] makes sense as using more classifiers constructs more fine-grained geoclasses via combinatorial partitioning and increases prediction resolution.
Note that the number of distinct partitions formed by {CPlaNet}[1-2] is 46,294 while it is 107,593 in CPlaNet[1-5].

The combinatorial partitioning of the proposed model is not limited to geoclass sets from our generation methods, but is generally applicable to any geoclass sets.
Therefore, we construct an additional instance of the proposed method, {CPlaNet}[1-5,PlaNet], which also incorporates PlaNet~(reprod), reproduced version of PlaNet model~\cite{weyand16planet} with our training data, additionally.
% in addition to the existing five base classifiers
% where PlaNet~(reprod) is a reproduced PlaNet~\cite{weyand16planet}.
{CPlaNet}[1-5,PlaNet] shows extra performance gains over {CPlaNet}[1-5] and achieves the state-of-the-art performance at all scales.
%In consequence, our models also outperform the previous approaches with more than 10 \% relative gains.
These experiments show that our combinatorial partitioning is a useful framework for image geolocalization through ensemble classification, where multiple classifiers with heterogeneous geoclass sets complement each other.



\iffalse
The geolocational accuracies of the proposed model on Im2GPS3k are shown in Table~\ref{tab:im2gps3k}.
%The geolocational accuracies of the proposed model on Im2GPS3k and YFCC4k are shown in Table~\ref{tab:im2gps3k} and~\ref{tab:yfcc4k}, respectively.
%Overall, the proposed models outperform the baselines and previous methods on these datasets and achieve the state-of-the art performance on Im2GPS at most of the scales.
Overall, the proposed models outperform the baselines and previous methods on these datasets at most of the scales.
%The magnitude differences of accuracies between the datasets come from the characteristics of the datasets.
%Images in Im2GPS are manually filtered to contain geolocational cues, and thus results in higher accuracies of the geolocalization.
%On the other hand, FlickrGeo is collected directly from the web without heavy filtering, and contains examples with very little geolocational information.
%Since images in the FlickrGeo dataset are collected from the web with minimal filtering and contain examples with little geolocational information, \eg, portraits without landmarks, improving accuracy is difficult.

%We analyze the models in depth mainly based on the FlickrGeo dataset hereafter because FlickrGeo is statistically more reliable for model analysis thanks to its large scale and better reflects the real-world image distribution.
%Note that the Im2GPS test set contains only 237 images and the results from the dataset are not likely to be statistically meaningful.
%The FlickrGeo test set, on the other hand, contains \textasciitilde14.5M images, \ie, it is 60K times larger than Im2GPS.






\subsubsection{Effects of Combinatorial Partitioning}
%Table~\ref{tab:flickrgeo} presents the performances of the models on FlickrGeo test set.
The models denoted by ClassSet~1 through 5 in Table~\ref{tab:flickrgeo} are trained with the geoclass sets generated from the parameters presented in Table~\ref{tab:geoclass}.
Using the learned models as the base classifiers, we construct two variants of the proposed method---CP[1-2] using the first two base classifiers and CP[1-5] using all the base classifiers, where CP denotes combinatorial partitioning.
%
%We train five classifiers (ClassSet~1 to ClassSet~5), each of which is trained with a geoclass set shown in Figure~\ref{fig:class_set}, and construct two instances of the proposed model: one with first two classifiers (Proposed[1-2]) and the other with all five classifiers (Proposed[1-5]).
As presented in Table~\ref{tab:flickrgeo}, both of our models outperform all the underlying classifiers at every scale.
Compared to the average of the underlying classifiers presented as Average[1-2] and Average[1-5], CP[1-5] shows \textasciitilde23 \% of accuracy gain at street level while CP[1-2] shows \textasciitilde19 \% improvement.
We emphasize that the proposed method achieves such large improvements while it does not involve any extra training but utilizes the results of the existing base classifiers;
This means that the geolocalization quality is improved through the combination process of merging individual results into fine-grained partitions.
Also, the larger improvement in CP[1-5] than in CP[1-2] is natural as more classifiers are used to ensemble, resulting in even more fine-grained geoclasses from the combinatorial partitioning.
Note that the number of distinct partitions formed by CP[1-2] is 46,294 while it is 107,593 in CP[1-5].
%The magnitude of the gains is most significant at the finest level while it is gradually reduced at coarser scales.
%Proposed~(1-5) shows \textasciitilde23 \% of accuracy gain at street level over the average accuracy of the underlying classifiers, \ie, Average~(1-5).
%This gain is larger than the one of Proposed~(1-2), which is \textasciitilde19 \%.
%The magnitude of the improvement is most significant at the finest level while it is gradually reduced at coarser scales.

The combinatorial partitioning of the proposed model is not limited to geoclass sets from our generation methods, but is generally applicable to any geoclass sets.
Therefore, we construct an additional instance of the proposed method, CP[1-5,PlaNet], which also incorporates PlaNet~(reprod) as a base classifier in addition to the five base classifiers where PlaNet~(reprod) is a reproduced PlaNet.
CP[1-5,PlaNet] shows extra performance gains over CP[1-5].
These experiments show that the combinatorial partitioning is a useful framework for image geolocalization through ensemble classification, where multiple classifiers with heterogeneous geoclass sets complement each other.
%Based on this observation, we believe that the combinatorial partitioning provides a framework where multiple classifiers with heterogeneous geoclass sets complement each other.
\fi




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\caption{Geolocational accuracies [\%] on YFCC4k.}
\label{tab:yfcc4k}
\scalebox{0.9}{
\begin{tabular}{
p{3.1cm}@{}|@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.5cm}@{}
}
Models	                                & 1~km	    & 5~km      & 10~km     & 25~km     & 50~km     & 100~km    & 200~km    & 750~km    & 2500~km	\\ \hline\hline
% [L] kNN,s=4. Numbers kindly provided by Nam Vo.
Deep-Ret~\cite{vo17revisiting}          & 2.3       & -         & -         & 5.7       & -         & -         & 11.0      & 23.5      & 42.0      \\
PlaNet (reprod)~\cite{weyand16planet}   & 5.6       & 10.1      & 12.2      & 14.3      &\bf{16.6}  &\bf{18.7}  & \bf{22.2} & \bf{36.4} & \bf{55.8} \\
CPlaNet[1-5]                                 & 7.3       & 11.7      & 13.1      &{14.7}     & 16.1      & 18.2      & 21.7      & 36.2      & 55.6      \\ 
CPlaNet[1-5,PlaNet]                          & \bf{7.9}  & \bf{12.1} & \bf{13.5} & \bf{14.8}  & 16.3     & 18.5      & 21.9      & \bf{36.4} & 55.5      \\
\hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\caption{Geolocational accuracies [\%] on Im2GPS.}
\label{tab:im2gps}
\scalebox{0.9}{
\begin{tabular}{
@{}p{0.1cm}@{}@{}p{0.3cm}@{}|p{3.0cm}@{}|@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.3cm}@{}
}
&&Models	                            & 1~km	        & 5~km      & 10~km     & 25~km     & 50~km     & 100~km    & 200~km    & 750~km    & 2500~km   \\ \hline\hline
&\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize{Retrieval}}}
 &Im2GPS~\cite{hays08im2gps}	        & - 	        & -         & -         & 12.0	    & -         & -         & 15.0	    & 23.0      & 47.0	    \\
&&Im2GPS~\cite{hays15large}	            & \phantom{0}2.5& 12.2      & 16.9      & 21.9      & 25.3      & 28.7      & 32.1      & 35.4      & 51.9      \\
&&Deep-Ret~\cite{vo17revisiting}	    & 12.2          & -         & -         & 33.3      & -         & -         & 44.3      & 57.4      & 71.3      \\
&&Deep-Ret+~\cite{vo17revisiting}	    & 14.4          & -         & -         & 33.3      & -         & -         & \bf{47.7} & 61.6      & 73.4      \\ \hline
&\multirow{6}{*}{\rotatebox[origin=c]{90}{\scriptsize{Classifier}}}
 &Deep-Cls~\cite{vo17revisiting}        & \phantom{0}6.8& -         & -         & 21.9      & -         & -         & 34.6      & 49.4      & 63.7  	\\
&&PlaNet~\cite{weyand16planet}          & \phantom{0}8.4& 19.0      & 21.5      & 24.5      & 27.8      & 30.4      & 37.6      & 53.6      & 71.3  	\\
&&PlaNet (reprod)~\cite{weyand16planet} & 11.0          & 23.6      & 26.6      & 31.2      & 35.4      & 30.5      & 37.6      & \bf{64.6} & \bf{81.9} \\ %\cline{3-12}
&&CPlaNet[1-2]	                            & 14.8          & 28.7      & 31.6      & 35.4      & 37.6      & 40.9      & 43.9      & 60.8      & 80.2      \\
&&CPlaNet[1-5]                               & 16.0          & \bf{29.1} & 33.3      & 36.7      & 39.7      & 42.2      & 46.4      & 62.4      & 78.5      \\
&&CPlaNet[1-5,PlaNet]                        & \bf{16.5}     & \bf{29.1} & \bf{33.8} & \bf{37.1} & \bf{40.5} & \bf{42.6} & 46.4      & 62.0      & 78.5      \\
\hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



We also present results on YFCC4k~\cite{vo17revisiting} dataset in Table~\ref{tab:yfcc4k}.
The overall tendency is similar to the one in Im2GPS3k.
Our full model outperforms Deep-Ret~\cite{vo17revisiting} consistently and significantly.
%It is noticeable that our model improves performance by 343\% and 142\% of the baseline accuracies at street level while still maintaining competitive scores at other scales.
The proposed algorithm also shows substantially better performance compared to PlaNet (reprod) in the low threshold range while two methods have almost identical accuracy at coarse-level evaluation.
%Note that the entire evaluation is more favorable to PlaNet (reprod) since our feature extractor is trained with PlaNet (reprod) classifier.


%\vspace{-0.2cm}
%\subsubsection{Evaluation on Im2GPS}
%Finally, we compare the proposed model with other existing methods on the Im2GPS test set in Table~\ref{tab:im2gps}.
%Compared to the existing methods, our model with two classifiers already achieves the best accuracies at the finest two levels and one with five classifiers even increases the performance gain as shown in Table~\ref{tab:im2gps}.
On the Im2GPS dataset, our model outperforms other classification-based approaches---Deep-Cls and PlaNet, which are single-classifier models with a different geoclass schema---significantly at every scale, as shown in Table~\ref{tab:im2gps}.
The performance of our models is also better than the retrieval-based models at most scales.
Moreover, our model, like other classification-based approaches, requires much less space than the retrieval-based models for inference.
%Table~\ref{tab:im2gps} shows that the quality of Deep-Ret is improved when the size of the database is increased in Deep-Ret+.
%However, this even worsens the space and time complexity of the model.
Although Deep-Ret+ improves Deep-Ret by increasing the size of the database, it even worsens space and time complexity.
In contrast, the classification-based approaches including ours do not require extra space when we have more training images.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
\centering
\begin{subfigure}[b]{0.9\linewidth}
\centering
\includegraphics[width=1\linewidth] {./figures/qualitative1.pdf}
\caption{Uluru in Australia}
\end{subfigure}

\begin{subfigure}[b]{0.9\linewidth}
\centering
\includegraphics[width=1\linewidth] {./figures/qualitative2.pdf}
\caption{Iao Needle in Hawaii}
\end{subfigure}
\caption{
Qualitative results of CPlaNet[1-5] on Im2GPS. 
Each map illustrates the progressive results of combinatorial partitioning by adding classifiers one by one.
S2 cells with the highest score and their centers are marked by green area and red pins respectively while the ground-truth location is denoted by the blue dots.
We also present the number of S2 cells in the highlighted region and distance between the ground-truth location and the center of the region in each map.
}
\label{fig:qualitative}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure~\ref{fig:qualitative} presents qualitative results of {CPlaNet}[1-5] on Im2GPS.
It shows how the combinatorial partitioning process improves the geolocalization quality.
Given an input image, each map shows an intermediate prediction as we accumulate the scores on different geoclass sets one by one.
The region with the highest score is progressively sharded into a smaller region with fewer S2 cells, and the center of the region gradually approaches to the ground-truth location as we integrate more classifiers for inference.

%Thus, we conduct an additional experiment incorporating PlaNet~(reprod) into the proposed model as one of the base classifiers;
%Proposed+PlaNet in Table~\ref{tab:flickrgeo} is the proposed model with six base classifiers: ClassSet~1 to ClassSet~5 and PlaNet~(reprod).


%Finally, Figure~\ref{fig:graph} presents the geolocalization accuracy of the proposed models and the base classifiers by continuously varying the radius $r$ in Eq.~\eqref{eq:geo_acc} up to the region scale.
%While there exist minor variations among the accuracies of base classifiers, we can observe a clear advantage by applying combinatorial partitioning.






\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering

\includegraphics[width=0.6\linewidth] {./figures/graph.pdf}

\caption{
Geolocational accuracies of proposed model and base classifiers measured by continuously varying geolocational radius $r$ in Eq.~\eqref{eq:geo_acc} up to region scale.
}
\label{fig:graph}
%\vspace{-0.1in}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\caption{Comparisons of numbers of distinct regions partitioned by two different models: single classifier model and proposed model.}
\label{tab:partitions}
\scalebox{0.8}{
\begin{tabular}{
@{}C{4cm}@{}|@{}C{2cm}@{}@{}C{2cm}@{}
}
    	                        & SingleSet	    & Proposed	        \\ \hline
Merging ClassSet 1-2	        & 19,938        & \phantom{0}46,294 \\
Merging ClassSet 1-5            & 55,007        & 107,593           \\ 
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi



%\subsubsection*{5.4.2 Computational Complexity  \vspace{0.3cm} \\ }
\subsubsection{Computational Complexity}
Although {CPlaNet} achieves competitive performance through combinatorial partitioning, one may be concerned about potential increase of time complexity for its inference due to additional classification layers and overhead in combinatorial partitioning process.
%Although our method increases the time complexity of the inference due to the extra classification layers and the combinatorial partitioning process, it is not a significant increase.
%However, it turns out that the extra computational cost is negligible as illustrated in Figure~\ref{fig:complexity} since adding few more classification layers on top of the shared feature extractor does not increase inference time substantially.
However, it turns out that the extra computational cost is negligible since adding few more classification layers on top of the shared feature extractor does not increase inference time substantially and the required information for combinatorial partitioning is precomputed as described in Section~\ref{sub:inference}.
Specifically, when we use 5 classification branches with combinatorial partitioning, theoretical computational costs for multi-head classification and combinatorial partitioning are only 2\% and 0.004\% of that of feature extraction process.
%Moreover, the combinatorial partitioning process only incurs linear increase of time complexity with respect to the number of the distinct partitions constructed by the partitioning.
%The additional complexity from combinatorial partitioning is negligible.
%Moreover, the combinatorial partitioning process only adds $O(N)$, where $N$ is the number of the distinct partitions constructed by the combinatorial partitioning.
In terms of space complexity, classification based methods definitely have great advantages over retrieval based ones, which need to maintain the entire image database.
Compared to a single-head classifier, our model with five base classifiers requires just four additional classification layers, which incurs moderate increase of memory usage.
%
\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth] {./figures/inference_complexity.pdf}
    \caption{
    Theoretical time complexity of inference with CP[1-5], which is measured by number of addtion and multiplication operations.
    Most computational cost for inference is from convolutional layers while classification and combinatorial partitioning have very minor impacts.
    %Note that the complexity for classification is still minor even though it sums up the complexities of five classification layers.
    }
    \label{fig:complexity}
\end{figure}
\fi




%\subsubsection*{5.4.3 Importance of Visual Features \vspace{0.3cm} \\}
\subsubsection{Importance of Visual Features}
%The number of geoclasses in ClassSet~1 and 2 is set to the number of classes in PlaNet~(reprod), wihch is determined by the adaptive geoclass generation in~\cite{weyand16planet}.
For geoclass set generation, all the parameters of ClassSet~1 and 2 are set to the same values except for the relative importance of two factors for edge weight definition; edge weights for ClassSet~1 are determined by visual distances only whereas those for ClassSet~2 are based on geolocational distances between the cells without any visual information of images.
%Despite the same parameters, 
ClassSet~1 presents better accuracies at almost all scales as in Table~\ref{tab:im2gps3k}.
This result shows how important visual information of images is when defining geoclass sets.

Moreover, we build another model (ImageNetFeat) learned with the same geoclass set with ClassSet~1 but using a different feature extractor pretrained on ImageNet~\cite{Deng09ImageNet}.
The large margin between ImageNetFeat and ClassSet~1 indicates importance of feature representation methods, and implies unique characteristics of visual cues required for image geolocalization compared to image classification.


\iffalse
We reproduce PlaNet, denoted by PlaNet~(reprod), and {\color{red}train the network with the adaptive geoclasses generated by setting the parameters as described in~\cite{weyand16planet}.
Unlike~\cite{weyand16planet}, where the center of an S2 cell is used as the center of a geoclass, we compute the center by averaging the GPS coordinates of training images in the geoclass as this technique improves the accuracies at fine scales as in the proposed model. [I don't think this sentence is good for us. It makes our contribution look trivial.]}
Note that the number of the geoclasses for ClassSet~1 and 2 is identical to the one in PlaNet~(reprod).
The street-level accuracy of ClassSet~1 is better than PlaNet~(reprod) while it is opposite at larger-scale levels.
%The performances of both ClassSet~1 and 2 outperform PlaNet~(reprod) at street level while it is opposite at larger-scale levels.
The high scores of PlaNet~(reprod) at large scales are achieved partly by dropping out regions with few images from the geoclass set by a predetermined threshold $t2$ in their adaptive partitioning.
Note that the fixed number of partitions are focused only on the regions that are not dropped; these regions can be partitioned more precisely.
%while the the number of geoclasses is fixed.
%Note that the remaining regions can be partitioned more by dropping out some regions while the total number of geoclasses is fixed.
However, a network trained on this geoclass set is never able to correctly predict the images outside of the regions.
Also, note that the parameters of the feature extractor are trained in PlaNet~(reprod) but not fine-tuned in ClassSet~1 and 2 implying that there are more rooms to improve the performances of our models.

ClassSet~2, in general, performs poorly compared to ClassSet~1 while the only difference of the generation parameters is the edge weights: the edge weights for ClassSet~1 are defined only by the visual distances of S2 cells whereas those for ClassSet~2 are defined by the geolocational distances only.
This result signifies the importance of visual features for the geoclass set generation.
%Based on the observation, we can choose different type of generation algorithms and our method is more suitable for applications requiring precise geolocalization.
\fi




\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\caption{Comparisons between the models with and without normalization for combinatorial partitioning on FlickrGeo.
The numbers of geoclasses for classifiers vary largely to highlight the effect of normalization.}
\label{tab:flickrgeo_normalization}
\scalebox{0.9}{
\begin{tabular}{
p{2.9cm}@{}|@{}C{1.3cm}@{}@{}C{1.3cm}@{}@{}C{1.35cm}@{}@{}C{1.45cm}@{}@{}C{1.65cm}@{}
}
Models	                        & Street 1~km	& City 25~km	& Region 200~km	& Country 750~km    & Continent 2500~km	\\ \hline\hline
ClassSet~1 (9969)	            & 4.8           & 11.6          & 20.6          & 36.9              & 56.5          	\\
ClassSet~2 (9969)	            & 4.3           & 11.7          & 20.5          & 36.8              & 56.4       	    \\
ClassSet~3 (3416)               & 1.7           & 10.8          & 20.1          & 36.6              & 56.1          	\\
ClassSet~4 (1444)               & 0.7           & \phantom{0}8.1& 18.6          & 35.8              & 55.0          	\\
ClassSet~5 (10600)              & 4.5           & 12.0          & 20.8          & 37.1              & \bf{56.7}        	\\ \hline
SimpleSum                       & 5.3           & 12.2          & 21.0          & 37.2              & 56.3          	\\
NormalizedSum                   & \bf{5.8}      & \bf{12.5}     & \bf{21.2}     & \bf{37.3}         & 56.6          	\\ \hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\caption{Comparisons between the models with and without normalization for combinatorial partitioning on Im2GPS3k.
Each number in parentheses denotes the geoclass set size, which varies largely to highlight the effect of normalization for this experiment.}
%\vspace{0.1cm}
\label{tab:flickrgeo_normalization}
\scalebox{0.9}{
\begin{tabular}{
p{2.7cm}@{}|@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.5cm}@{}
}
Models              & 1~km      & 5~km      & 10~km	    & 25~km     & 50~km     & 100~km    & 200~km    & 750~km    & 2500~km   \\ \hline\hline
ClassSet~1  (9969)  & 8.4       & 18.3      & 21.7      & 24.7      & 27.4      & 29.8      & 34.1      & 47.9      & 64.5      \\
ClassSet~2  (9969)  & 8.0       & 17.6      & 20.6      & 23.8      & 26.2      & 29.2      & 32.7      & 46.6      & 63.9      \\
ClassSet~3 (3416)   & 4.2       & 15.9      & 19.1      & 22.8      & 24.9      & 28.0      & 31.4      & 46.1      & 63.5      \\
ClassSet~4 (1444)   & 1.8       & 9.5       & 13.2      & 16.8      & 21.2      & 24.5      & 29.5      & 44.4      & 61.8      \\
ClassSet~5 (10600)  & 8.2       & 19.1      & 22.3      & 25.2      & 27.3      & 29.9      & 33.6      & 47.3      & \bf{65.5} \\ \hline
SimpleSum           & 9.7       & 19.4      & 23.1      & 26.6      & 28.1      & 30.6      & 33.8      & 47.7      & 64.0      \\
NormalizedSum       & \bf{9.8}  & \bf{19.8} & \bf{23.6} & \bf{26.8} & \bf{28.8} & \bf{31.1} & \bf{34.9} & \bf{48.3} & 65.0      \\ \hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\subsubsection*{5.4.4 Classifier balancing \vspace{0.3cm} \\}
\subsubsection{Balancing Classifiers}
We normalize the scores assigned to individual S2 cells as discussed in Section~\ref{sub:inference}, which is denoted by NormalizedSum, to address the artifact that sums of all S2 cell scores are substantially different across classifiers.
To highlight the contribution of NormalizedSum, we conduct an additional experiment with classsets that have large variations in number of classes.
Table~\ref{tab:flickrgeo_normalization} presents that NormalizedSum clearly outperforms the combinatorial partitioning without normalization (SimpleSum) while SimpleSum still illustrates competitive accuracy compared to the base classifiers.

\iffalse
To investigate the effect of balancing classifier scores introduced in Section~\ref{sub:inference}, we conduct more experiments 
%with a different variation of geoclass sets.
%In this setting, 
for which we replace the three randomly generated geoclass sets with another three randomly generated ones whose number of geoclasses vary substantially, while we keep the first two geoclass sets. % with manually designed parameters.
Table~\ref{tab:flickrgeo_normalization} presents the results from this experiment, where each number in parentheses denotes the geoclass set size.% of a classifier.
When we apply the combinatorial partitioning without normalization (SimpleSum), the quality of the geolocalization is still improved compared to the base classifiers.
%However, such model does not gain much accuracy with respect to CP[1-2] in Table~\ref{tab:im2gps3k}, which is identical to the combination of the first two classifiers in this new setting; indeed, the street-level accuracy is even lower than CP[1-2].
The performance gain is further improved by NormalizedSum using a proper normalization technique.
%the performance increase becomes more significant at every scale compared to SimpleSum when applying the normalization to the combinatorial partitioning (NormalizedSum).}
\fi







\iffalse
\begin{table}
\centering
\caption{Results on Im2GPS test set.}
\label{tab:im2gps}
\scalebox{0.8}{
\begin{tabular}{
@{}p{0.1cm}@{}@{}p{0.4cm}@{}|p{2.4cm}@{}|@{}C{1.3cm}@{}@{}C{1.3cm}@{}@{}C{1.35cm}@{}@{}C{1.45cm}@{}@{}C{1.65cm}@{}
}
&&Models	                        & Street 1~km	& City 25~km	& Region 200~km	& Country 750~km    & Continent 2500~km	\\ \hline
&\multirow{4}{*}{\rotatebox[origin=c]{90}{Retrieval}}
 &Im2GPS~\cite{hays08im2gps}	    &   	        & 12.0	        & 15.0	        & 23.0              & 47.0	            \\
&&Im2GPS~\cite{hays15large}	        & \phantom{0}2.5& 21.9          & 32.1          & 35.4              & 51.9          	\\
&&Deep-Ret~\cite{vo17revisiting}	& 12.2          & 33.3          & 44.3          & 57.4              & 71.3          	\\
&&Deep-Ret+~\cite{vo17revisiting}	& 14.4          & 33.3          & 47.7          & 61.6              & 73.4          	\\ \hline
&\multirow{9}{*}{\rotatebox[origin=c]{90}{Classification}}
 &Deep-Cls~\cite{vo17revisiting}    & \phantom{0}6.8& 21.9          & 34.6          & 49.4              & 63.7          	\\
&&PlaNet~\cite{weyand16planet}      & \phantom{0}8.4& 24.5          & 37.6          & 53.6              & 71.3          	\\
&&PlaNet~(reprod)                   & 11.0          & 31.7          & \bf{51.1}     & \bf{65.0}         & 77.6          	\\ 
&&ImageNetFeat	                    & \phantom{0}5.5& 13.1          & 19.8          & 25.7              & 51.1          	\\ \cline{3-8}
&&ClassSet~1	                    & 13.5          & 33.3          & 46.0          & 63.3              & 79.8          	\\
&&ClassSet~2	                    & 12.7          & \bf{37.1}     & 45.6          & 61.6              & \bf{80.6}       	\\
&&ClassSet~3	                    & 13.5          & 35.4          & 48.1          & 61.2              & 77.2          	\\
&&ClassSet~4	                    & 13.9          & 34.2          & 47.3          & 63.7              & 78.5          	\\
&&ClassSet~5	                    & 14.8          & 36.3          & 46.4          & 60.8              & 77.6          	\\ \cline{3-8}
&&Proposed (1-2)	                & 14.8          & 35.4          & 43.9          & 60.8              & 80.2          	\\
&&Proposed (1-5)                    & \bf{16.0}     & 36.4          & 46.4          & 62.5              & 78.5          	\\ 
\end{tabular}
}
\end{table}
\fi



%%%%%%%%%%

\iffalse
%\vspace{-0.35cm}
\paragraph{Performance issues [R1, R2]}
%Jack
While our algorithm does not improve baseline approaches at coarse levels (country and continent), the motivation of combinatorial partitioning is to improve the accuracy at fine-grained levels (street and city) which is generally more important.
%Although our algorithm does not outperform other approaches consistently in all levels, we believe that the accuracy at fine-grained levels (street and city) is more important.
%The area of correct answers has the diameter of 50 km already in city-level, which allows large errors.
According to Table~2, our full model (CP[1-5,PlaNet]) obtains 35\% and 22\% relative gains from PlaNet and from individual classifiers respectively at street level.
Figure~\ref{fig:graph} shows that our method outperforms all base classifiers consistently and significantly at street and city levels.
%While the ranks of the base classifiers change at different point of x-axis, the proposed method consistently shows the best performance at every point.
%
%the graph of geolocational accuracies varying the allowable error up to city-level.
%
These improvements are statistically significant as we tested on a very large test set.
\fi





\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{./rebuttal/rebut_figs/graph.pdf}
\caption{
Geolocational accuracies on FlickrGeo varying the allowable error up to city-level (lower lines are better).
}
\label{fig:graph}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi




==> ECCV 2018 (CP) Camera Ready/sections/introduction.tex <==
% !TEX root = ../main.tex

%%%%%%%%% BODY TEXT
\section{Introduction}
\label{sec:introduction}

%\hsseo{(Intro. to image geolocalization)}
Image geolocalization is the task of predicting the geographic location of an image based only on its pixels without any meta-information.
As the geolocation is an important attribute of an image by itself, it also plays as a proxy to other location attributes such as elevation, weather, and distance to a particular point of interest.
However, geolocalizing images is a challenging task since input images often contain limited visual information representative of their locations.
To handle this issue effectively, the model is required to capture and maintain visual cues of the globe comprehensively.

%\hsseo{(Two main streams: retrieval vs. classification)}
There exist two main streams to address this task: retrieval and classification based approaches.
The former searches for nearest neighbors in a database of geotagged images by matching their feature representations~\cite{hays08im2gps,hays15large,vo17revisiting}.
Visual appearance of an image at a certain geolocation is estimated using the representations of the geotagged images in database.
The latter treats the task as a classification problem by dividing the map into multiple discrete classes~\cite{vo17revisiting,weyand16planet}.
Thanks to recent advances in deep learning, simple classification techniques based on convolutional neural networks handle such complex visual understanding problems effectively.
%Unlike retrieval based techniques, this approach does not require to maintain a database of geotagged images for inference.
%Instead, geographic visual information needs to be represented by a set of model parameters learned from training.

%\hsseo{(Advantages of classification model)}
There are several advantages of formulating the task as classification instead of retrieval.
First, classification-based approaches save memory and disk space to store information for geolocalization; they just need to store a set of model parameters learned from training images whereas all geotagged images in the database should be embedded and indexed to build retrieval-based systems.
In addition to space complexity, inference of classification-based approaches is faster because a result is given by a simple forward pass computation of a deep neural network while retrieval-based methods undergo significant overhead for online search from a large index given a query image.
Finally, classification-based algorithms provide multiple hypotheses of geolocation with no additional cost by presenting multi-modal answer distributions.
%Finally, classification based algorithms naturally express multi-modal answer distributions, which provides rich information useful for post-processing and algorithm analysis.

%\hsseo{(limitations of classification model)}
On the other hand, the standard classification-based approaches have a few critical limitations.
They typically ignore correlation of spatially adjacent or proximate classes.
%Geolocation classes, which are the output of the classifier, are treated all distinct regardless of their inter-distance on maps.
For instance, assigning a photo of Bronx to Queens, which are both within New York city, is treated equally wrong as assigning it to Seoul.
Another drawback comes from artificially converting continuous geographic space into discrete class representations.
Such an attempt may incur various artifacts since images near class boundaries are not discriminative enough compared to data variations within classes; training converges slowly and 
%classification 
performance is affected substantially by subtle changes in map partitioning.
This limitation can be alleviated by increasing the number of classes and reducing the area of the region corresponding to each class.
However, this strategy increases the number of parameters while decreasing the size of the training dataset per class.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
%\includegraphics[width=0.5\linewidth]{figures/combinatorial_partitioning.pdf}
\includegraphics[width=0.8\linewidth]{figures/combinatorial_partitioning_wide.pdf}
\caption{
Visualization of combinatorial partitioning. 
Two coarse-grained class sets, $\mathcal{P}=\{p_1,p_2,\dots,p_5\}$ and $\mathcal{Q}=\{q_1,q_2,\dots,q_5\}$ in the map on the left, are merged to construct a fine-grained partition as shown in the map on the right by a combination of geoclasses in the two class sets.
%It forms a fine-grained partitioning as shown in the map on the top.  
Each resulting fine-grained class is represented by a tuple $(p_i, q_j)$, and is constructed by identifying partially overlapping partitions in $\mathcal{P}$ and $\mathcal{Q}$.
%The partition with the highest score is used for the final prediction.
%Maps with black boundary show the partitioned regions by geo-classes and color intensity illustrates magnitude of scores.
%Scores over multiple geoclasses, $\mathcal{P}=\{p_1,p_2,\dots,p_5\}$ and $\mathcal{Q}=\{q_1,q_2,\dots,q_5\}$ (bottom maps) are merged at every intersection between geoclasses of multiple sets forming a fine-grained partitioning (top map).
}
%\vspace{-0.3cm}
\label{fig:comb_part}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
discretizations introduce upper-bounds of the model by predicting the identical geolocation for images assigned to the same class.
Although the upper-bounds can be mitigated by increasing the number of output classes, it is not always easy as it will increase the number of parameters linearly.
Moreover, the training example per each class will be reduced as the number of classes increases and it will end up with an equivalent of the retrieval based model when the number of classes becomes equal to the number of examples in the dataset.
\fi

%\hsseo{(How we manage to overcome these limitations)}
To overcome such limitations, we propose a novel algorithm that enhances the resolution of geoclasses and avoids the training data deficiency issue.
This is achieved by \emph{combinatorial partitioning}, which is a simple technique to generate spatially fine-grained classes through a combination of the multiple configurations of classes.
This idea has analogy to product quantization~\cite{jegou11product} since they both construct a lot of quantized regions using relatively few model parameters through a combination of low-bit subspace encodings or coarse spatial quantizations.
Our combinatorial partitioning allows the model to be trained with more data per class by considering a relatively small number of classes at a time.
Figure~\ref{fig:comb_part} illustrates an example of combinatorial partitioning, which enables generating more classes with minimal increase of model size and learning individual classifiers reliably without losing training data per class.
Combinatorial partitioning is applied to an existing classification-based image geolocalization technique, PlaNet~\cite{weyand16planet}, and our algorithm is referred to as CPlaNet hereafter.
%When there are two different class definitions, the final prediction is made on a new set of classes, which is given by a combination of two configurations.
%Such combination leads to generate more classes with minimal increase of model size, and makes it possible to learn individual classifiers reliably without losing training data per class.
%We train multiple classifiers on different geo-class sets that are generated by differently merging initial regions.
%Given the predictions from each classifier, the predicted score of a geo-class is added to the score of its corresponding region.
%Since all geo-class sets have different geolocational boundaries on maps, the region of a geo-class is partitioned into multiple sub-regions, which are intersections with classes in other geo-class sets; 
%the geolocation is then predicted based on more finely subdivided regions working around the aforementioned issues as depicted in Figure~\ref{fig:comb_part}.
%
%\hsseo{(Our contribution)}
Our contribution is threefold:
\begin{itemize}
    \item[$\bullet$] We introduce a novel classification-based model for image geolocalization using combinatorial partitioning, which defines a fine-grained class configuration by combining multiple heterogeneous geoclass sets in coarse levels.
    \item[$\bullet$] We propose a technique that generates multiple geoclass sets by varying parameters, and design an efficient inference technique to combine prediction results from multiple classifiers with proper normalization.
    %\item We propose a technique that generates multiple geoclass sets by varying parameters, and show that \hsseo{models with generated geoclass sets perform as well as the one with the adaptive partitioning in~\cite{weyand16planet}.}
    %\item We propose a technique that generates multiple geoclass sets by mutating parameters, and show that a properly generated geoclass set alone improves the performance effectively.
    \item[$\bullet$] The proposed algorithm outperforms the existing techniques in multiple benchmark datasets, especially at fine scales.
    %\item[$\bullet$] We present an inference technique appropriate for classification-based image geolocalization and achieve improved performance in multiple benchmark datasets especially at fine scales.
\end{itemize}

%\hsseo{(Paper organization)}
The rest of this paper is organized as follows. 
We review the related work in Section~\ref{sec:rel_work}, and describe combinatorial partitioning for image geolocalization in Section~\ref{sec:comb_part}.
The details about training and inference procedures are discussed in Section~\ref{sec:learning}.
We present experimental results of our algorithm in Section~\ref{sec:exp}, and conclude our work in Section~\ref{sec:conclusion}.

==> ECCV 2018 (CP) Camera Ready/sections/learning.tex <==
% !TEX root = ../main.tex

\section{Learning and Inference}
\label{sec:learning}
This section describes more details about CPlaNet including network architecture, and training and testing procedure.
We also discuss data structures and the detailed inference algorithm. 

\subsection{Network Architecture}
\label{sub:training}
Following \cite{weyand16planet}, we construct our network based on the Inception architecture~\cite{szegedy2015going} with batch normalization~\cite{szegedy2016rethinking}.
Inception v3 without the final classification layer (\texttt{fc} with \texttt{softmax}) is used as our feature extractor, and multiple branches of classification layers are attached on top of the feature extractor as illustrated in Figure~\ref{fig:net_arch}.
We train the multiple classifiers independently while keeping the weights of the Inception module fixed.
% Model parameter sizes in bytes (incl batch norm params):
% all 40 heads: 2355161580
% avg head: 58879039.5
% whole model: 2442372724
% feature extractor: 87211144
%
% Inference times (average of 30 inferences):
% Feature extractor only: 0.11s
% Feature extractor + Head 0: 0.12s
% Feature extractor + Head 0-4: 0.13s
Note that, since all classifiers share the feature extractor, our model requires marginal increase of memory to maintain multiple classifiers.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{figures/network_architecture.pdf}
\caption{
Network architecture of our model. 
A single Inception v3 architecture is used as our feature extractor after removing the final classification layer.
An image feature is fed to multiple classification branches and classification scores are predicted over multiple geoclass sets.
}
\label{fig:net_arch}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Inference with Multiple Classifiers}
\label{sub:inference}
Once the predicted scores in each class set are assigned to the corresponding regions, the subregions overlapped by multiple class sets are given cumulated scores from multiple classifiers.
%After this procedure, we select the partition with the highest score and compute its center as the final prediction of geolocation.
%{\color{red} [We need some equations to formally describe inference procedure here.]}
%
%\subsection{Balancing impacts of classifiers}
%\label{sec:sub:norm}
A simple strategy to accumulate geoclass scores is to add the scores to individual S2 cells within the geoclass.
Such a simple strategy is inappropriate since it gives favor to classifiers that have geoclasses corresponding to large regions covering more S2 cells.
To make each classifier contribute equally to the final prediction regardless of its class configuration, we normalize the scores from individual classifiers with consideration of the number of S2 cells per class before adding them to the current S2 cell scores.
Formally, given a geoclass score distributed to S2 cell $g_k$ within a class in a geoclass set $\mathcal{C}^i$, denoted by $\mathrm{geoscore}(g_k; \mathcal{C}^i)$, an S2 cell is given a score $s(\cdot)$ by
%Formally, given a function of S2 cell $g_k$ and a geoclass set $\mathcal{C}^i$ with a geoclass score output, denoted by $\mathrm{geoscore}(\cdot, \cdot)$, the score of an S2 cell $s(g_k)$ is given by
\begin{equation}
    \label{eq:norm}
    s(g_k) = \sum_{i=1}^{N}{\frac{\mathrm{geoscore}(g_k; \mathcal{C}^i)}{\sum_{t=1}^{K}{\mathrm{geoscore}(g_t; \mathcal{C}^i)}}},
\end{equation}
where $K$ is the total number of S2 cells and $N$ is the number of geoclass sets.
Note that this process implicitly creates fine-grained partitions because the regions defined by different geoclass combinations are given different scores.

After this procedure, we select the S2 cells with the highest scores and compute their center for the final prediction of geolocation by averaging locations of images in the S2 cells. 
That is, the predicted geolocation $l_\mathrm{pred}$ is given by
%
\iffalse
\begin{align}
    \mathcal{G} &= \argmax_{k}{s(g_k)} \\
    l_\mathrm{pred} &= \ddfrac{\sum_{k \in \mathcal{G}}{\sum_{e \in g_k}{\mathrm{geolocation}\left(e\right)}}}{\sum_{k \in \mathcal{G}}{\left| g_k \right|}} 
    \label{eq:prediction}
\end{align}
\fi
%
\begin{equation}
%    l_\mathrm{pred} = \ddfrac{\sum_{k \in \mathcal{G}}{\sum_{e \in g_k}{\mathrm{geolocation}\left(e\right)}}}{\sum_{k \in \mathcal{G}}{\left| g_k \right|}},
    l_\mathrm{pred} = \frac{\sum_{k \in \mathcal{G}}{\sum_{e \in g_k}{\mathrm{geolocation}\left(e\right)}}}{\sum_{k \in \mathcal{G}}{\left| g_k \right|}},
    \label{eq:prediction}
\end{equation}
%
%{\color{red}[have to redefine $g_\mathrm{max}$ since it can be multiple s2 cells.]}
where $\mathcal{G} = \argmax_{k}{s(g_k)}$ is an index set of the S2 cells with the highest scores and $\mathrm{geolocation}(\cdot)$ is a function to return the ground-truth GPS coordinates of a training image $e$.
Note that an S2 cell $g_k$ may contain a number of training examples.

In our implementation, all fine-grained partitions are precomputed offline by generating all existing combinations of the multiple geoclass sets, and an index mapping from each geoclass to its corresponding partitions is also constructed offline to accelerate inference.
Moreover, we precompute the center of images in each partition.
%for faster inference after the geoclass sets are generated.
%In our implementation, 
To compute the center of a partition, we convert the latitude and longitude values of GPS tags into 3D Cartesian coordinates.
This is because a na\"ive average of latitude and longitude representations introduces significant errors as the target locations become distant from the equator.
%\hsseo{When adapting 3D Cartesian coordinates, we can omit the denominator in Eq.~\eqref{eq:prediction} as the any vectors having the same direction represent the same location on the earth surface, where the vector penetrates.}


\iffalse
\subsection{Implementation Details for Inference}
{\color{red} [This subsection is almost redundant.]}
%\hsseo{(Our particular implementation)}
For implementation of the inference procedure with combinatorial partitioning, we define multiple geoclass sets by uniquely merging locally connected S2 cells at a certain level as described in Section~\ref{sec:sub:geo_gen}. 
\hsseo{
As we maintain the region for a geoclass using a set of S2 cells,
our model assigns a score of each geoclass to its corresponding S2 cells after normalization described by Eq.~\eqref{eq:norm}.
}
Since each geoclass set covers the entire earth, every S2 cell gets a score from each classifier and the scores of an S2 cell obtained from multiple classifiers are accumulated.
Finally, our model selects the locally connected S2 cells with the highest accumulated scores, and computes the center by averaging\footnote{Because a simple average of latitude and longitude values introduces large errors near polar regions, we convert latitudes and longitudes into 3D Cartesian coordinates, average them, and convert the result back to latitude and longitude space.} the S2 cell centers weighted by number of training images contained in individual cells.
Note that the center of each S2 cell is precomputed by averaging the locations of training images within the cell.
\fi




==> ECCV 2018 (CP) Camera Ready/sections/related_work.tex <==
% !TEX root = ../main.tex

%%%%%%%%% BODY TEXT
\section{Related Work}
\label{sec:rel_work}

%
% Geolocalization by classification
%
%This work is based on PlaNet \cite{weyand16planet}, which formulates image geolocalization problem as a classification task. 
%
%\cite{Wang17Corr} classify photo of person into one of 12 cities using CNN
%
%
% Geolocalization by retrieval
%
The most common approach of image geolocalization is based on the image retrieval pipeline. 
Im2GPS \cite{hays08im2gps,hays15large} and its derivative~\cite{vo17revisiting} perform image retrieval in a database of geotagged images using global image descriptors. 
%A recent extension of im2GPS \cite{vo17revisiting} replaces hand-crafted features by the activations of a classification CNN similar to PlaNet, and presents improved accuracy.
%We briefly review the classification based geolocalization methods.
%
Various visual features can be applied to the image retrieval step.
NetVLAD~\cite{Arandjelovic16CVPR} is a global image descriptor trained end-to-end for place recognition on street view data using a ranking loss. 
Kim et al.~\cite{Kim17CVPR} learn a weighting mask for the NetVLAD descriptor to focus on image regions containing location cues. 
%
While global features have the benefit to retrieve diverse natural scene images based on ambient information, local image features yield higher precision in retrieving structured objects such as buildings and are thus more frequently used~\cite{Baatz10ECCV,Cao15IJCV,Chen11CVPR,Kim15ICCV,Knopp10ECCV,Philbin07CVPR,Schindler07CVPR,Zamir10ECCV,Zamir14PAMI}. 
DELF~\cite{Noh17ICCV} is a deeply learned local image feature detector and descriptor with attention for image retrieval.

On the other hand, classification-based image geolocalization formulates the problem as a classification task. 
In~\cite{vo17revisiting,weyand16planet}, a classifier is trained to predict the geolocation of an input image.
Since the geolocation is represented in a continuous space, classification-based approaches quantize the map of the entire earth into a set of geoclasses corresponding to partitioned regions.
Note that training images are labeled into the corresponding geoclasses based on their GPS tags.
At test time, the center of the geoclass with the highest score is returned as the predicted geolocation of an input image.
This method is lightweight in terms of space and time complexity compared to retrieval-based methods, but its prediction accuracy highly depends on how the geoclass set is generated.
Since every image that belongs to the same geoclass has an identical predicted geolocation, more fine-grained partitioning is preferable to obtain precise predictions.
However, it is not always straightforward to increase the number of geoclasses as it linearly increases the number of parameters and makes the network prone to overfitting to training data.


%
% geometric pose estimation
%
Pose estimation approaches~\cite{Cao15IJCV,Irschara09CVPR,Li10ECCV,Li12ECCV,Liu17ICCV,Sattler11ICCV,Sattler12BMVC} match  query images against 3D models of an area, and employ 2D-3D feature correspondences to identify 6-DOF query poses. 
Instead of directly matching against a 3D model, \cite{Sattler17CVPR,Sattler12BMVC} first perform image retrieval to obtain coarse locations and then estimate poses using the retrieved images.
%
%
% deep pose estimation
%
%Instead of geometrically solving for pose, 
PoseNet~\cite{Kendall17CVPR,Kendall15ICCV} treats pose estimation as a regression problem based on a convolutional neural network.
The accuracy of PoseNet is improved by introducing an intermediate LSTM layer for dimensionality reduction~\cite{Walch17ICCV}.

%
% Landmark recognition
%
A related line of research is landmark recognition, where images are clustered by their geolocations and visual similarity to construct a database of popular landmarks.
The database serves as the index of an image retrieval system~\cite{Avrithis10MM,Gammeter09ICCV,Johns11ICCV,Quack08CIVR,Zheng09CVPR,Weyand15CVIU} or the training data of a landmark classifier~\cite{Bergamo13CVPR,Li09CVPR,Gronat13CVPR}.
%
%
% cross-view geolocalization
%
Cross-view geolocation recognition makes additional use of satellite or aerial imagery to determine query locations~\cite{Workman15ICCV,Lin13CVPR,Lin15CVPR,Tian17CVPR}.


==> ECCV 2018 (CP) Camera Ready/tables.tex <==
% !TEX root = main.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\caption{Geolocational accuracies [\%] on Im2GPS.}
\label{tab:im2gps}
\scalebox{0.8}{
\begin{tabular}{
@{}p{0.1cm}@{}@{}p{0.3cm}@{}|p{2.5cm}@{}|@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.3cm}@{}
}
&&Models	                        & 1~km	        & 5~km      & 10~km     & 25~km     & 50~km     & 100~km    & 200~km    & 750~km    & 2500~km   \\ \hline\hline
&\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize{Retrieval}}}
 &Im2GPS~\cite{hays08im2gps}	    & - 	        & -         & -         & 12.0	    & -         & -         & 15.0	    & 23.0      & 47.0	    \\
&&Im2GPS~\cite{hays15large}	        & \phantom{0}2.5& 12.2      & 16.9      & 21.9      & 25.3      & 28.7      & 32.1      & 35.4      & 51.9      \\
&&Deep-Ret~\cite{vo17revisiting}	& 12.2          & -         & -         & 33.3      & -         & -         & 44.3      & 57.4      & 71.3      \\
&&Deep-Ret+~\cite{vo17revisiting}	& 14.4          & -         & -         & 33.3      & -         & -         & 47.7      & 61.6      & 73.4      \\ \hline
&\multirow{6}{*}{\rotatebox[origin=c]{90}{\scriptsize{Classifier}}}
 &Deep-Cls~\cite{vo17revisiting}    & \phantom{0}6.8& -         & -         & 21.9      & 34.6      & -         & -         & 49.4      & 63.7  	\\
&&PlaNet[org]~\cite{weyand16planet} & \phantom{0}8.4& 19.0      & 21.5      & 24.5      & 27.8      & 30.4      & 37.6      & 53.6      & 71.3  	\\ %\cline{3-8}
&&PlaNet[rep]~\cite{weyand16planet} & 11.0          & 23.6      & 26.6      & 31.2      & 35.4      & 30.5      & 37.6      & \bf{64.6} & \bf{81.9} \\ %\cline{3-8}
&&CP[1-2]	                        & 14.8          & -         & -         & 35.4      & -         & -         & 43.9      & 60.8      & 80.2      \\
&&CP[1-5]                           & \bf{16.0}     & \bf{29.1} & \bf{33.3} & \bf{36.7} & 39.7      & 42.2      & 46.4      & 62.4      & 78.5      \\
&&CP[1-5,PlaNet]                    & 13.9          & 26.2      & 28.7      & 35.4      & \bf{41.8} & \bf{43.0} & \bf{48.5} & 62.4      & 78.9      \\
\hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\caption{Geolocational accuracies [\%] on YFCC4k.}
\label{tab:yfcc4k}
\scalebox{0.9}{
\begin{tabular}{
p{2.3cm}@{}|@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.3cm}@{}
}
Models	                        & 1~km	    & 5~km      & 10~km     & 25~km     & 50~km     & 100~km    & 200~km    & 750~km    & 2500~km	\\ \hline\hline
% [L] kNN,s=4. Numbers kindly provided by Nam Vo.
Deep-Ret~\cite{vo17revisiting}  & 2.3       & -         & -         & 5.7       & -         & -         & 11.0      & 23.5      & 42.0      \\
PlaNet (reprod)                 & 5.6       & 10.1      & 12.2      & 14.3      &\bf{16.6}  &\bf{18.7}  & \bf{22.2} & \bf{36.4} & \bf{55.8} \\
CP[1-5]                         & 7.3       & 11.7      & 13.1      &{14.7}     & 16.1      & 18.2      & 21.7      & 36.2      & 55.6       	\\ 
CP[1-5,PlaNet]                  & \bf{7.9}  & \bf{12.1} & \bf{13.5} & \bf{14.8}  & 16.3     & 18.5      & 21.9      & \bf{36.4} & 55.5     \\
\hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\caption{Geolocational accuracies [\%] on Im2GPS3k.}
\label{tab:im2gps3k}
\scalebox{0.9}{
\begin{tabular}{
p{2.3cm}@{}|@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.3cm}@{}
}
Models	                        & 1~km	    & 5~km      & 10~km     & 25~km     & 50~km     & 100~km    & 200~km    & 750~km    & 2500~km	\\ \hline\hline
Deep-Ret~\cite{vo17revisiting}  & 7.2       & -         & -         & 19.4      & -         & -         & 26.9      & 38.9      & 55.9      \\
PlaNet (reprod)                 & 8.5       & 18.1      & 21.4      & 24.8      & 27.7      & 30.0      & 34.3      & 48.4      & \bf{64.6} \\
CP[1-5]                         & 9.9       & 20.2      & 23.3      & 26.3      & 28.5      & 30.4      & 34.5      & \bf{48.8} & \bf{64.6} \\ 
CP[1-5,PlaNet]                  & \bf{10.2} & \bf{20.8} & \bf{23.7} & \bf{26.5} & \bf{28.6} & \bf{30.6} & \bf{34.6} & 48.6      & \bf{64.6} \\
\hline
\end{tabular}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables.tex <==
% !TEX root = main.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\caption{Geolocational accuracies [\%] on Im2GPS.}
\label{tab:im2gps}
\scalebox{0.8}{
\begin{tabular}{
@{}p{0.1cm}@{}@{}p{0.3cm}@{}|p{2.5cm}@{}|@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.3cm}@{}
}
&&Models	                        & 1~km	        & 5~km      & 10~km     & 25~km     & 50~km     & 100~km    & 200~km    & 750~km    & 2500~km   \\ \hline\hline
&\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize{Retrieval}}}
 &Im2GPS~\cite{hays08im2gps}	    & - 	        & -         & -         & 12.0	    & -         & -         & 15.0	    & 23.0      & 47.0	    \\
&&Im2GPS~\cite{hays15large}	        & \phantom{0}2.5& 12.2      & 16.9      & 21.9      & 25.3      & 28.7      & 32.1      & 35.4      & 51.9      \\
&&Deep-Ret~\cite{vo17revisiting}	& 12.2          & -         & -         & 33.3      & -         & -         & 44.3      & 57.4      & 71.3      \\
&&Deep-Ret+~\cite{vo17revisiting}	& 14.4          & -         & -         & 33.3      & -         & -         & 47.7      & 61.6      & 73.4      \\ \hline
&\multirow{6}{*}{\rotatebox[origin=c]{90}{\scriptsize{Classifier}}}
 &Deep-Cls~\cite{vo17revisiting}    & \phantom{0}6.8& -         & -         & 21.9      & 34.6      & -         & -         & 49.4      & 63.7  	\\
&&PlaNet[org]~\cite{weyand16planet} & \phantom{0}8.4& 19.0      & 21.5      & 24.5      & 27.8      & 30.4      & 37.6      & 53.6      & 71.3  	\\ %\cline{3-8}
&&PlaNet[rep]~\cite{weyand16planet} & 11.0          & 23.6      & 26.6      & 31.2      & 35.4      & 30.5      & 37.6      & \bf{64.6} & \bf{81.9} \\ %\cline{3-8}
&&CP[1-2]	                        & 14.8          & -         & -         & 35.4      & -         & -         & 43.9      & 60.8      & 80.2      \\
&&CP[1-5]                           & \bf{16.0}     & \bf{29.1} & \bf{33.3} & \bf{36.7} & 39.7      & 42.2      & 46.4      & 62.4      & 78.5      \\
&&CP[1-5,PlaNet]                    & 13.9          & 26.2      & 28.7      & 35.4      & \bf{41.8} & \bf{43.0} & \bf{48.5} & 62.4      & 78.9      \\
\hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\caption{Geolocational accuracies [\%] on YFCC4k.}
\label{tab:yfcc4k}
\scalebox{0.9}{
\begin{tabular}{
p{2.3cm}@{}|@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.3cm}@{}
}
Models	                        & 1~km	    & 5~km      & 10~km     & 25~km     & 50~km     & 100~km    & 200~km    & 750~km    & 2500~km	\\ \hline\hline
% [L] kNN,s=4. Numbers kindly provided by Nam Vo.
Deep-Ret~\cite{vo17revisiting}  & 2.3       & -         & -         & 5.7       & -         & -         & 11.0      & 23.5      & 42.0      \\
PlaNet (reprod)                 & 5.6       & 10.1      & 12.2      & 14.3      &\bf{16.6}  &\bf{18.7}  & \bf{22.2} & \bf{36.4} & \bf{55.8} \\
CP[1-5]                         & 7.3       & 11.7      & 13.1      &{14.7}     & 16.1      & 18.2      & 21.7      & 36.2      & 55.6       	\\ 
CP[1-5,PlaNet]                  & \bf{7.9}  & \bf{12.1} & \bf{13.5} & \bf{14.8}  & 16.3     & 18.5      & 21.9      & \bf{36.4} & 55.5     \\
\hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\caption{Geolocational accuracies [\%] on Im2GPS3k.}
\label{tab:im2gps3k}
\scalebox{0.9}{
\begin{tabular}{
p{2.3cm}@{}|@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.2cm}@{}@{}C{1.3cm}@{}
}
Models	                        & 1~km	    & 5~km      & 10~km     & 25~km     & 50~km     & 100~km    & 200~km    & 750~km    & 2500~km	\\ \hline\hline
Deep-Ret~\cite{vo17revisiting}  & 7.2       & -         & -         & 19.4      & -         & -         & 26.9      & 38.9      & 55.9      \\
PlaNet (reprod)                 & 8.5       & 18.1      & 21.4      & 24.8      & 27.7      & 30.0      & 34.3      & 48.4      & \bf{64.6} \\
CP[1-5]                         & 9.9       & 20.2      & 23.3      & 26.3      & 28.5      & 30.4      & 34.5      & \bf{48.8} & \bf{64.6} \\ 
CP[1-5,PlaNet]                  & \bf{10.2} & \bf{20.8} & \bf{23.7} & \bf{26.5} & \bf{28.6} & \bf{30.6} & \bf{34.6} & 48.6      & \bf{64.6} \\
\hline
\end{tabular}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
